How the Experts Algorithm Can Help Solve LPs Online

We consider the problem of solving packing/covering LPs online, when the columns of the constraint matrix are presented in random order. This problem has received much attention and the main focus is to figure out how large the right-hand sides of the LPs have to be (compared to the entries on the left-hand side of the constraints) to allow $(1+\epsilon)$-approximations online. It is known that the right-hand sides have to be $\Omega(\epsilon^{-2} \log m)$ times the left-hand sides, where $m$ is the number of constraints. In this paper we give a primal-dual algorithm that achieve this bound for mixed packing/covering LPs. Our algorithms construct dual solutions using a regret-minimizing online learning algorithm in a black-box fashion, and use them to construct primal solutions. The adversarial guarantee that holds for the constructed duals helps us to take care of most of the correlations that arise in the algorithm; the remaining correlations are handled via martingale concentration and maximal inequalities. These ideas lead to conceptually simple and modular algorithms, which we hope will be useful in other contexts.

==> solvingRandomLP.tex <==

\section{Solving Random LPs}
\label{sec:random-lps}

\agnote{Drop this section.}
% \agnote{Make notation consistent. I am using the old notation from the
%   only-LP writeup. We should clarify that we know the value of $n$ when
%   we are given a random LP.}

% \begin{thm}
%   \label{thm:one-phase}
%   Let $\e \leq 1/20$, and $\delta \in (0,\e)$. Given a $c$-slack LP $\L
%   \in \PLPn$ for $c \geq 326$, suppose the columns are presented to us
%   in uniformly random order. Let $\L_1, \L_2$ be the LPs obtained by
%   restricting to columns in the first and second halves of this random
%   ordering. We can find an online solution to the LP $\L_2$ with value
%   at least
%   \[ (1 - O(\e))\, \OPT(\L_2) - O(\e\, \OPT(\L)) \]
%   with probability at least $1 - O(\delta)$. 
% \end{thm}

% \begin{proof}
%   Let $S$ be the set of columns of $\L$ that appear in the second half
%   of the random permutation, and let LP $\L_2 := \L^S$ be the resulting
%   LP.  Since $S$ a random $(n/2)$-subset of $[n]$, we can use these
%   columns to get estimates $\btau, \bOhat, \bbhat$ that satisfy the
%   properties in Theorem~\ref{thm:est-lp-params} with probability $1 -
%   O(\delta/m)$. Let us condition on this good event.

%   The algorithm is simple: we pick all items in $S$ with values greater
%   than threshold $\btau$.  Let $H := \{ t \in S: \pi_t > \btau\}$ be
%   these ``high'' valued elements. This leaves the residual LP $\L_2(val
%   \leq \btau)$. On this residual LP we run the algorithm \LPtoLB from
%   Theorem~\ref{thm:LPAssEstimates}. 

%   By property~(1) of goodness, we know that $\OPT(\L_2(val \leq \btau))
%   + \sum_{t \in H} \pi_t \geq (1 - \e) \OPT(\L_2)$. So if $\sum_{t \in
%     H} \pi_t \geq (1- 161\e) \OPT(\L_2)$, we can ignore the value of
%   items picked by \LPtoLB: just the elements
%   of $H$ give us enough value to satisfy the statement of the
%   theorem. (We can ensure that \LPtoLB never violates the
%   capacities $\RHS(\L_2(val \leq \btau))$, which means we always have
%   enough space to add in all items of $H$.)  \agnote{Do we want to
%     say more than this?} Else we know that $\OPT(\L_2(val \leq \btau))
%   \geq 160\e\, \OPT(\L_2)$. Now we can assume that $\OPT(\L_2)
%   \geq 100\e\, \OPT(\L)$, else returning a solution of value zero would
%   satisfy the claim of the theorem. For the rest of this proof we assume
%   both these conditions hold, so that $\OPT(\L_2(val \leq \btau)) \geq
%   16000\e^2\, \OPT(\L)$.

%   We need to pass the algorithm \LPtoLB several estimates and parameters.
%   First, let us see how the parameter $\gamma$ of
%   Theorem~\ref{thm:LPAssEstimates} behaves.
%   \begin{gather}
%     \gamma = \max \left\{ \max_{i \in [m], t \in S}
%       \frac{a_{it}}{\RHS(\L_2(val \leq \btau))_i}, \max_{t \in S}
%       \frac{\pi_t}{\OPT(\L_2(val \leq \btau))} \right\} \leq \max
%     \left\{ \max_{i \in [m]} \frac{(1+\e)}{\bbhat_i},
%       \frac{\btau}{\bOhat} \right\}. \label{eq:gam}
%   \end{gather}
%   If we define $\bgamma$ to be the expression on the right, and set $\e'
%   := \max \{ \e, \sqrt{ \bgamma \log (m/\delta)} \}$. By definition it
%   satisfies $\bgamma \leq \e'^2/(\log (m/\delta))$. Since $\e' \geq \e$,
%   we get that $\delta \leq \e'$.

%   To show that $\e' \leq 1/10$, first we bound $\bgamma$: by
%   property~(2) of goodness, we know that $\RHS(\L_2(val \leq \btau))
%   \geq (c/4)B \ones$, and hence the first term of the maximum
%   in~(\ref{eq:gam}) is at most $1/B$. By property~(3) of goodness, the
%   second term in~(\ref{eq:gam}) is at most $\frac{160 \OPT(\L_2)}{B
%     \cdot \OPT(\L_2(val \leq \btau))}$. So
%   \begin{gather}
%     \e' \leq \e \max\left\{1 , \sqrt{\frac{160\, \OPT(\L_2)}{\OPT(\L_2(val
%         \leq \btau))}} \right\}. \label{eq:eps-prime}
%   \end{gather}
%   Finally, using that $\OPT(\L_2(val \leq \btau)) \geq 16000\e^2\,
%   \OPT(\L)$, we can infer that $\e' \leq 1/10$. \agnote{need to prove
%     the lower bound of $\sqrt{\log (m/\e)/n}$ on $\e'$ as well.}

%   We now pass to \LPtoLB the
%   estimates on the optimal value $\bOhat \in [\OPT(\L_2(val \leq \btau))
%   - O(\e B\btau), \OPT(\L_2(val \leq \btau))]$, the estimates for the
%   right hand side $\bbhat \in \RHS(\L_2(val \leq \btau)) (1 \pm \e)$,
%   $\e'$, $\delta$, the number of columns $n/2$, and the number of
%   constraints $m$.  And what do we get back? We get a solution for
%   $\L_2(val \leq \btau)$ with value at least
%   \[ (1 - 16\e')\, \OPT(\L_2(val \leq \btau)) - O(\e B \btau) \] with
%   probability $1 - \delta$.  Adding in the items from $H$ that we picked
%   on the side, and using the value of $\e'$ from~(\ref{eq:eps-prime}),
%   we have a solution of value
%   \begin{align*}
%     & \sum_{t \in H} \pi_t + \OPT(\L_2(val \leq \btau)) - O(\e)
%     \sqrt{\OPT(\L) \cdot \OPT(\L_2(val \leq \btau))} - O(\e B \btau) \\
%     & \geq  (1 - \e) \OPT(\L_2) - O(\e) \OPT(\L) \quad \geq \quad
%     \OPT(\L_2) - O(\e) \OPT(\L)
%   \end{align*}
%   as claimed. 
% \end{proof}

% In expectation, $\OPT(\L_2) = \frac12 \OPT(\L)$, so this shows we get a
% solution to the second half of the columns comparable to expected value
% of the second half, which is only about $\frac12 - \e$ of the entire
% LP. To get better, we now apply this idea recursively.

\subsection{Many Phases}

Consider the random LP $\L$ with $n$ columns, and define several sets:
for $i = 0,1,\ldots, \log \e^{-1}$, the $i^{th}$ set $S_i$ contains the
first $2^i \e n$ columns. Consider $\L^{S_i}$, whose RHS is scaled down
to $\RHS(\L) \cdot \frac{|S_i|}{n} = \RHS(\L) \cdot \frac{\e 2^i}{n}$.
%Let $T = \{0, 1, \ldots, \log \e^{-1}\}$.
Assume $\L$ is $c$-slack for $c$ sufficiently large. For each $i \in
\{0,1, \ldots, \log \e^{-1}\}$, define $\e_i = \e \cdot
\smash{\sqrt{\frac{n}{|S_i|}}}$, so that $\e_i = \sqrt{\e/2^i}$. Note
that the restricted LPs $\L^{S_i}$ are also $c$-slack, but with respect
to an altered value of $B$, namely $B_i = \frac{\log
  (m/\delta)}{\e_i^2}$. Moreover, by the doubling sizes of the sets
$S_i$, note that the sets $S_i \setminus S_{i-1}$ for $i \geq 1$ are
disjoint, and partition the columns in $(\e n, 1]$.

We can apply Theorem~\ref{thm:one-phase} to each $\L^i$ for $i \geq
1$ to get a solution to the LP $\L^{S_i \setminus S_{i-1}}$ of value 
\[ \OPT(\L^{S_i \setminus S_{i-1}}) - O(\e_i) \OPT(\L^{S_i}). \] with
probability at least $1 - O(\delta)$. These solutions are for disjoint
sets of columns, and by the way we altered the right hand sides of the
LP, all of these feasible solutions can be simultaneously packed into
the original RHSs with probability $1 - O(T\delta)$ using a trivial
union bound. The value of this LP is 
\[ \sum_{i \geq 1} \OPT(\L^{S_i \setminus S_{i-1}}) - \sum_{i \geq 1}
O(\e_i) \OPT(\L^{S_i}). \]

First, the terms being subtracted: by Lemma~\ref{lemma:expected-PLP}(i)
we know that $E[\OPT(\L^{S_i})] \leq \e 2^i \OPT(\L)$. Hence, the
expectation of the sum being subtracted is
\begin{gather}
  \sum_{i = 1}^{(\log \e^{-1})} \e_i \left( \e 2^i \OPT(\L) \right) =
  \e^{3/2} \OPT(\L) \sum_{i = 1}^{(\log \e^{-1})} \sqrt{ 2^{-i} } =
  \Theta(\e\, \OPT(\L)). \label{eq:sum-errs}
\end{gather}

Now, to lower bound $\sum_{i \geq 1} \OPT(\L^{S_i \setminus
  S_{i-1}})$. Define $T_i := S_i \setminus S_{i-1}$. Fix an $i \geq 1$,
and let $\bx$ be a optimal solution for $\L$, and let $\bx^{(i)}$ be the
solution scaled down by $(1 - \e_i)$ and restricted to the $2^{i-1} \e
n$ columns in $T_i$. To be a solution to $\L^{T_i}$, we want $\sum_{t
  \in T_i} \ba_t \bx^{(i)}_t \leq 2^{i-1} \e \bb$. Note that $E[\sum_{t
  \in T_i} \ba_t \bx^{(i)}_ t] \leq (1 - \e_i)2^{i-1} \e \bb$, and
$\L$ being $c$-slack means that $\bb \geq c B \ones$. Hence, the chance
of the sum of these vectors exceeding their expectation is at most
\[ \sum_{j = 1}^m \exp\left\{ - \frac{ (\e_i \cdot \e 2^{i-1} b_i)^2 }{
    4 \e 2^{i-1} b_i } \right\} = \sum_{j = 1}^m \exp\left\{ - \frac{
    \e_i^2 \cdot \e 2^{i-1} b_i }{ 4 } \right\} \leq \sum_{j = 1}^m
\exp\left\{ - \frac{ \e^2 b_i }{ 8 } \right\}. \] Using $b_i \geq cB$
for $c \geq 16$ gives this probability is at most $\delta^2/m$. Define
the good event $\mathcal{G}$ if any of the solutions $\bx^{(i)}$ is
infeasible for $\L^{T_i}$ in any of the $\log \e^{-1}$ phases; we get
$\Pr[\mathcal{G}] \geq 1 - (\log \e^{-1}) \delta^2/m$ by a union
bound. Observe that for each sample point $\omega$ in $\mathcal{G}$, the
solution is just a scaled down version of $\bx$, and hence
\[ \sum_{i \geq 1} \OPT(L^{T_i}) \geq \pi^T \bx - \sum_{i \geq 0} \e_i
\sum_{t \in T_i(\omega)} \bpi_t \bx_t. \]
Here we have defined $\e_0 = 1$ for convenience.
Now, since $\OPT(\cdot)$ is non-negative, we get
\[ \E \left[ \sum_{i \geq 1} \OPT(\L^{T_i}) \right] \geq \E \left[ \sum_{i
    \geq 1} \OPT(\L^{T_i}) \,\middle|\, \mathcal{G} \right] \Pr[
\mathcal{G} ] 
\geq \pi^T \bx \cdot  \Pr[\mathcal{G}] - \E\left[ \sum_{i \geq 0} \e_i
\sum_{t \in T_i} \bpi_t \bx_t \,\middle|\, \mathcal{G} \right] \cdot \Pr[\mathcal{G}] .\]
Moreover, again by the non-negativity of the $\bpi_t \bx_t$ terms, we get
\[ 
\E\left[ \sum_{i \geq 0} \e_i \sum_{t \in T_i} \bpi_t \bx_t \right] \geq
\E\left[ \sum_{i \geq 0} \e_i \sum_{t \in T_i} \bpi_t \bx_t \,\middle|\,
  \mathcal{G} \right] \cdot \Pr[\mathcal{G}] \] Putting the two
together, and using $\OPT(\L) = \pi^T \bx$, we have
\[ \E \left[ \sum_{i \geq 1} \OPT(\L^{T_i}) \right] \geq \OPT(\L) \cdot
\Pr[\mathcal{G}] - \E\left[ \sum_{i \geq 0} \e_i \sum_{t \in T_i} \bpi_t
  \bx_t \right]. \] The rest is immediate: $\E[ \sum_{t \in T_i} \bpi_t
\bx_t ] = (\e 2^i) \OPT(\L)$, and hence
\[ \E\left[ \sum_{i \geq 0} \e_i \sum_{t \in T_i} \bpi_t \bx_t \right] =
\sum_{i \geq 0} \e_i (\e 2^i) \OPT(\L). \] This last calculation is the
same as~(\ref{eq:sum-errs}) apart from inclusion of the term $i = 0$,
but the result is again $O(\e) \OPT(\L)$. 

Putting it all together, the expected value is at least $(1 - O(\e))
\OPT(\L)$ with probability $1 - O(\delta)$. (This relies on parameters
that ensure that $(\log \e^{-1}) \delta^2/m \leq O(\e)$.

